Constraints on Deep-seated Zonal Winds Inside Jupiter and Saturn

The atmospheres of Jupiter and Saturn exhibit strong and stable zonal winds. How deep the winds penetrate unabated into each planet is unknown. Our investigation favors shallow winds. It consists of two parts. The first part makes use of an Ohmic constraint; Ohmic dissipation associated with the planet's magnetic field cannot exceed the planet's net luminosity. Application to Jupiter (J) and Saturn (S) shows that the observed zonal winds cannot penetrate below a depth at which the electrical conductivity is about six orders of magnitude smaller than its value at the molecular-metallic transition. Measured values of the electrical conductivity of molecular hydrogen yield radii of maximum penetration of 0.96R_J and 0.86R_S, with uncertainties of a few percent of R. At these radii, the magnetic Reynolds number based on the zonal wind velocity and the scale height of the magnetic diffusivity is of order unity. These limits are insensitive to difficulties in modeling turbulent convection. They permit complete penetration along cylinders of the equatorial jets observed in the atmospheres of Jupiter and Saturn. The second part investigates how deep the observed zonal winds actually do penetrate. Truncation of the winds in the planet's convective envelope would involve breaking the Taylor-Proudman constraint on cylindrical flow. This would require a suitable nonpotential acceleration which none of the obvious candidates appears able to provide. Accelerations arising from entropy gradients, magnetic stresses, and Reynolds stresses appear to be much too weak. These considerations suggest that strong zonal winds are confined to shallow, stably stratified layers, with equatorial jets being the possible exception.

==> macros.tex <==
\hyphenation{mix-ing ben-zene naph-tha-lene north-ern path-ways}
\hyphenation{phen-an-threne photo-chemical at-mo-spheres}  

\newcommand{\chh}{\mbox{CH$_2$}}
\newcommand{\tom}{\stackrel{\rm M}{\longrightarrow}}
\newcommand{\toh}{\stackrel{h\nu}{\longrightarrow}}
\newcommand{\brx}{\begin{reaction}}
\newcommand{\nrx}{\end{reaction}}

\newenvironment{reaction}{\begin{tabbing}
\hspace*{1.0in}\=\hspace{4.0in}\=number \kill}
	{\end{tabbing}}

\newenvironment{netreaction}{\begin{tabbing}
\hspace*{0.50in}\=\hspace{0.50in}\=\hspace{4.0in}\=number \kill}
	{\end{tabbing}}

\newenvironment{rate}{\begin{tabbing}
\hspace*{1.25in}\=rate \kill}
	{\end{tabbing}}

%\let\jnl@style=\rmfamily
%\def\ref@jnl#1{{\jnl@style#1}}%
\newcommand\aj{\ref@jnl{AJ}}% 
          % Astronomical Journal 
\newcommand\araa{\ref@jnl{ARA\&A}}% 
          % Annual Review of Astron and Astrophys 
\newcommand\apj{\ref@jnl{ApJ}}% 
          % Astrophysical Journal 
\newcommand\apjl{\ref@jnl{ApJ}}% 
          % Astrophysical Journal, Letters 
\newcommand\apjs{\ref@jnl{ApJS}}% 
          % Astrophysical Journal, Supplement 
\newcommand\ao{\ref@jnl{Appl.~Opt.}}% 
          % Applied Optics 
\newcommand\apss{\ref@jnl{Ap\&SS}}% 
          % Astrophysics and Space Science 
\newcommand\aap{\ref@jnl{A\&A}}% 
          % Astronomy and Astrophysics 
\newcommand\aapr{\ref@jnl{A\&A~Rev.}}% 
          % Astronomy and Astrophysics Reviews 
\newcommand\aaps{\ref@jnl{A\&AS}}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand\azh{\ref@jnl{AZh}}% 
          % Astronomicheskii Zhurnal 
\newcommand\baas{\ref@jnl{BAAS}}% 
          % Bulletin of the AAS 
\newcommand\jrasc{\ref@jnl{JRASC}}% 
          % Journal of the RAS of Canada 
\newcommand\memras{\ref@jnl{MmRAS}}% 
          % Memoirs of the RAS 
\newcommand\mnras{\ref@jnl{MNRAS}}% 
          % Monthly Notices of the RAS 
\newcommand\pra{\ref@jnl{Phys.~Rev.~A}}% 
          % Physical Review A: General Physics 
\newcommand\prb{\ref@jnl{Phys.~Rev.~B}}% 
          % Physical Review B: Solid State 
\newcommand\prc{\ref@jnl{Phys.~Rev.~C}}% 
          % Physical Review C 
\newcommand\prd{\ref@jnl{Phys.~Rev.~D}}% 
          % Physical Review D 
\newcommand\pre{\ref@jnl{Phys.~Rev.~E}}% 
          % Physical Review E 
\newcommand\prl{\ref@jnl{Phys.~Rev.~Lett.}}% 
          % Physical Review Letters 
\newcommand\pasp{\ref@jnl{PASP}}% 
          % Publications of the ASP 
\newcommand\pasj{\ref@jnl{PASJ}}% 
          % Publications of the ASJ 
\newcommand\qjras{\ref@jnl{QJRAS}}% 
          % Quarterly Journal of the RAS 
\newcommand\skytel{\ref@jnl{S\&T}}% 
          % Sky and Telescope 
\newcommand\solphys{\ref@jnl{Sol.~Phys.}}% 
          % Solar Physics 
\newcommand\sovast{\ref@jnl{Soviet~Ast.}}% 
          % Soviet Astronomy 
\newcommand\ssr{\ref@jnl{Space~Sci.~Rev.}}% 
          % Space Science Reviews 
\newcommand\zap{\ref@jnl{ZAp}}% 
          % Zeitschrift fuer Astrophysik 
\newcommand\nat{\ref@jnl{Nature}}% 
          % Nature 
\newcommand\iaucirc{\ref@jnl{IAU~Circ.}}% 
          % IAU Cirulars 
\newcommand\aplett{\ref@jnl{Astrophys.~Lett.}}% 
          % Astrophysics Letters 
\newcommand\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}% 
          % Astrophysics Space Physics Research 
\newcommand\bain{\ref@jnl{Bull.~Astron.~Inst.~Netherlands}}% 
          % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{\ref@jnl{Fund.~Cosmic~Phys.}}% 
          % Fundamental Cosmic Physics 
\newcommand\gca{\ref@jnl{Geochim.~Cosmochim.~Acta}}% 
          % Geochimica Cosmochimica Acta 
\newcommand\grl{\ref@jnl{Geophys.~Res.~Lett.}}% 
          % Geophysics Research Letters 
\newcommand\jpc{\ref@jnl{J.~Phys.~Chem.}}% 
          % Journal of Physical Chemistry 
\newcommand\jcp{\ref@jnl{J.~Chem.~Phys.}}% 
          % Journal of Chemical Physics 
\newcommand\jgr{\ref@jnl{J.~Geophys.~Res.}}% 
          % Journal of Geophysics Research 
\newcommand\memsai{\ref@jnl{Mem.~Soc.~Astron.~Italiana}}% 
          % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{\ref@jnl{Nucl.~Phys.~A}}% 
          % Nuclear Physics A 
\newcommand\physrep{\ref@jnl{Phys.~Rep.}}% 
          % Physics Reports 
\newcommand\physscr{\ref@jnl{Phys.~Scr}}% 
          % Physica Scripta 
\newcommand\planss{\ref@jnl{Planet.~Space~Sci.}}% 
          % Planetary Space Science 
\newcommand\procspie{\ref@jnl{Proc.~SPIE}}% 
          % Proceedings of the SPIE 

\def\jj{{\mathbf{J}}}
\def\bu{{\mathbf{U}}}
\def\uu{{\mathbf{U}}}
\def\blu{{\mathbf{u}}}
\def\bup{{\mathbf{U}_P}}
\def\but{{\mathbf{U}_T}}
\def\bb{{\mathbf{B}}}
\def\blb{{\mathbf{b}}}
\def\bbp{{\mathbf{B}_P}}
\def\bbt{{\mathbf{B}_T}}

\def\br{{\mathbf{r}}}
\def\ba{{\mathbf{A}}}
\def\bj{{\mathbf{J}}}
\def\be{{\mathbf{E}}}
\def\bff{{\mathbf{F}}}
\def\bn{{\mathbf{\nabla}}}

\newcommand{\Tesla}{\ \rm{Tesla}}
\newcommand{\Km}{\ \rm{Km}}
\newcommand{\m}{\ \rm{m}}
\newcommand{\cm}{\ \rm{cm}}
\newcommand{\s}{\ \rm{s}}
\newcommand{\W}{\ \rm{W}}
\newcommand{\K}{\ \rm{K}}
\newcommand{\bigS}{\ \rm{S}}
\newcommand{\bigs}{\ \rm{S}}
\newcommand{\g}{\ \rm{g}}
\newcommand{\Kg}{\ \rm{Kg}}
\newcommand{\mathbar}{\ \rm{bar}}
\newcommand{\Mbar}{\ \rm{Mbar}}
\newcommand{\G}{\ \rm{G}}
\newcommand{\J}{\ \rm{J}}
\newcommand{\A}{\ \rm{A}}
\newcommand{\erg}{\ \rm{erg}}


\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\de}{\partial}
\newcommand{\er}{\mathbf{e}_r}
\newcommand{\et}{\mathbf{e}_{\theta}}
\newcommand{\ep}{\mathbf{e}_{\phi}}
\newcommand{\ez}{\mathbf{e}_{z}}
\newcommand{\ey}{\mathbf{e}_{y}}
\newcommand{\ex}{\mathbf{e}_{x}}

%\newcommand\slantfrac{\case}% 
%\newcommand\onehalf{\slantfrac{1}{2}}% 
%\newcommand\onethird{\slantfrac{1}{3}}% 
%\newcommand\twothirds{\slantfrac{2}{3}}% 
%\newcommand\onequarter{\slantfrac{1}{4}}% 
%\newcommand\threequarters{\slantfrac{3}{4}}% 
%\newcommand\ubvr{\mbox{$U\!BV\!R$}}%% UBVR system 
%\newcommand\ub{\mbox{$U\!-\!B$}}%   % U-B 
%\newcommand\bv{\mbox{$B\!-\!V$}}%   % B-V 
%\newcommand\vr{\mbox{$V\!-\!R$}}%   % V-R 
%\newcommand\ur{\mbox{$U\!-\!R$}}%   % U-R 
%\newcommand\ion[2]{#1$\;${\small\rmfamily\@Roman{#2}}\relax}% 
%\newcommand\nodata{ ~$\cdots$~ }% 
%\newcommand\diameter{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}% 
\newcommand\arcdeg{\mbox{$^\circ$}}
\newcommand\degr{\arcdeg}

